Investigating Vulnerability to Adversarial Examples on Multimodal Data Fusion in Deep Learning

The success of multimodal data fusion in deep learning appears to be attributed to the use of complementary in-formation between multiple input data. Compared to their predictive performance, relatively less attention has been devoted to the robustness of multimodal fusion models. In this paper, we investigated whether the current multimodal fusion model utilizes the complementary intelligence to defend against adversarial attacks. We applied gradient based white-box attacks such as FGSM and PGD on MFNet, which is a major multispectral (RGB, Thermal) fusion deep learning model for semantic segmentation. We verified that the multimodal fusion model optimized for better prediction is still vulnerable to adversarial attack, even if only one of the sensors is attacked. Thus, it is hard to say that existing multimodal data fusion models are fully utilizing complementary relationships between multiple modalities in terms of adversarial robustness. We believe that our observations open a new horizon for adversarial attack research on multimodal data fusion.

==> table/Table_1.tex <==
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\begin{table}[!t]
	\renewcommand{\arraystretch}{1.0}
	\centering
	\caption{Dice and Jaccard coefficient comparison of our approach and six different approaches on PH2 + ISBI 2016 Challenge dataset.}
	\vspace{0.2cm}
	\resizebox{0.999\linewidth}{!}{
	\begin{tabular}{M{3.5cm}M{2.9cm}M{2.9cm}}
		\toprule \toprule
		\textbf{Method}          & \textbf{Dice Coefficient} & \textbf{Jaccard Coefficient} \\ \toprule \toprule
		SCDRR \cite{32}        & 86.00            & 76.00              \\
		JCLMM \cite{33}          & 82.85            & -              \\
		MSCA \cite{34}          & 81.57            & 72.33              \\
		SSLS \cite{35}          & 78.38            & 68.16              \\
		FCN \cite{10}            & 89.40            & 82.15               \\
		Bi et al. (2017) \cite{25}  & 90.66            & 83.99               \\ \midrule
		\textbf{\makecell{FCN+BPB+SBE \\ (Our method)}} & \textbf{91.84}            & \textbf{84.30}              \\ \bottomrule
	\end{tabular}}
	\vspace{0.1cm}
\end{table}


==> table/Table_2.tex <==
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\begin{table}[!t]
	\renewcommand{\arraystretch}{1.0}
	\centering
	\caption{Dice and Jaccard coefficient comparison of our approach and conventional segmentation network on TVUS dataset.}
	\vspace{0.2cm}
	\resizebox{0.999\linewidth}{!}{
	\begin{tabular}{M{3.5cm}M{2.9cm}M{2.9cm}}
		\toprule \toprule
		\textbf{Method}          & \textbf{Dice Coefficient} & \textbf{Jaccard Coefficient} \\ \toprule \toprule
		U-Net \cite{6}        & 82.30            & 70.38              \\
		FCN \cite{10}         & 81.19            & 69.12              \\
		Dilated-Net \cite{19}         & 82.40            & 70.36              \\
		Park et al. (2019) \cite{40} & 82.67            & 70.46               \\ \midrule
		\textbf{Dilated-Net+BPB+SBE \newline(Our method)} & \textbf{83.52}            & \textbf{71.58}              \\ \bottomrule
	\end{tabular}}
	\vspace{-0.1cm}
\end{table}


==> table/Table_3.tex <==
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\begin{table}[!t]
	\renewcommand{\arraystretch}{1.0}
	\centering
	\caption{Statistical significance analysis of performance improvements by paired t-test on PH2+ISBI 2016 dataset.}
	\vspace{0.2cm}
	\resizebox{0.999\linewidth}{!}{
		\begin{tabular}{M{2.5cm}M{2.5cm}M{1.8cm}M{1.5cm}}
			\toprule \toprule
			 \textbf{Baseline Network}          & \makecell{\textbf{Mean difference}\\$\pm$\\   \textbf{Standard Error}} & \textbf{95\% CI} & \textbf{\textit{p}-value} \\ \toprule \toprule
			U-Net \cite{6}            & 1.22$\pm$0.21                                                                                         & {[} 0.51, 1.35{]} & p\textless{}0.0001 \\
			FCN \cite{10}             & 2.17$\pm$0.28                                                                                         & {[}1.41, 2.72 {]} & p\textless{}0.0001 \\
			Dilated-Net \cite{19}     & 2.03$\pm$0.25                                                                                         & {[}1.34, 2.46{]}  & p\textless{}0.0001
			\\ \bottomrule
		\end{tabular}}
		\vspace{-0.1cm}
\end{table}


==> table/Table_4.tex <==
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\begin{table}[!t]
	\renewcommand{\arraystretch}{1.0}
	\centering
	\caption{Statistical significance analysis of performance improvements by paired t-test on TVUS dataset.}
	\vspace{0.2cm}
	\resizebox{0.999\linewidth}{!}{
		\begin{tabular}{M{2.5cm}M{2.5cm}M{1.8cm}M{1.5cm}}
			\toprule \toprule
		\textbf{Baseline Network}          & \makecell{\textbf{Mean difference}\\$\pm$\\   \textbf{Standard Error}} & \textbf{95\% CI} & \textbf{\textit{p}-value} \\ \toprule \toprule
			U-Net \cite{6}           & 0.92$\pm$0.13                                                                                         & {[} 0.66, 1.17{]} & p\textless{}0.0001 \\
			FCN \cite{10}             & 1.62$\pm$0.28                                                                                         & {[}1.07, 2.17{]} & p\textless{}0.0001 \\
			Dilated-Net \cite{19}     & 0.90$\pm$0.11                                                                                         & {[}0.62, 1.1{]}   & p\textless{}0.0001
			\\ \bottomrule
	\end{tabular}}
	\vspace{-0.2cm}
\end{table}

